Is It a Trap? A Large-scale Empirical Study And Comprehensive Assessment of Online Automated Privacy Policy Generators for Mobile Apps

Privacy regulations protect and promote the privacy of individuals by requiring mobile apps to provide a privacy policy that explains what personal information is collected and how these apps process this information. However, developers often do not have sufficient legal knowledge to create such privacy policies. Online Automated Privacy Policy Generators (APPGs) can create privacy policies, but their quality and other characteristics can vary. In this paper, we conduct the first large-scale empirical study and comprehensive assessment of APPGs for mobile apps. Specifically, we scrutinize 10 APPGs on multiple dimensions. We further perform the market penetration analysis by collecting 46,472 Android app privacy policies from Google Play, discovering that nearly 20.1% of privacy policies could be generated by existing APPGs. Lastly, we point out that generated policies in our study do not fully comply with GDPR, CCPA, or LGPD. In summary, app developers must carefully select and use the appropriate APPGs with careful consideration to avoid potential pitfalls.

==> 9_DataAvailability.tex <==
\vspace{-8pt}
\section{Data Availability}
\vspace{-3pt}
The \textbf{``Crawled Privacy Policy Collection''} is available at: 

\noindent https://github.com/APPG-APPG/APPG. This work involves significant data collection and engineering effort. We hope the reviewers understand our need to reserve the source code and some raw data for the submission. We will release the full replication package on paper acceptance.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Tables/name.tex <==
  \begin{tabular}{l|cccccccccc}
    \toprule
    \textbf{Data Right} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10  \\
\midrule
     Right to Access &\cmark &\xmark &\cmark &\cmark &\xmark &\xmark &\cmark &\cmark &\cmark&\cmark\\
\midrule
    Right to Rectify or Erase &\cmark&\xmark &\cmark &\cmark &\xmark &\xmark&\cmark &\cmark &\cmark &\cmark\\
\midrule
    Right to Restrict of Processing &\cmark &\xmark &\cmark &\cmark &\xmark &\xmark &\cmark &\cmark &\cmark&\xmark\\
    
\midrule
    Right to Object to Processing  &\cmark &\xmark &\cmark &\cmark &\xmark &\xmark &\cmark &\cmark &\cmark&\xmark\\
\midrule
    Right to Data Portability &\cmark &\xmark &\cmark &\cmark &\xmark &\xmark &\cmark &\cmark &\cmark&\xmark\\
\midrule 
    Right to Lodge a Complaint &\cmark &\xmark &\cmark &\cmark &\xmark &\xmark &\cmark &\cmark &\cmark&\cmark\\
  \bottomrule
\end{tabular}

==> omitted_PrivacyRegulation.tex <==
\section{Privacy Regulation}
\label{sec_introduction_legal}

Most mobile apps will collect personal information, collect data from mobile phone sensors, and/or share data with third-party services. So, privacy policies are important to clarify the usage of data and related behaviours, and are required and enacted in various jurisdictions.
We manually examined five well-known bodies of privacy regulation for personal information and privacy protection, from the European Union (European General Data Protection Regulation, GDPR)~\cite{GDPR}, the United States (California Consumer Privacy Act, CCPA)~\cite{CCPA}, Brazil (Law of General Data Protection, LGPD)~\cite{LGPD}, Australia (Australian Privacy Principles, APP)~\cite{APPs} and China (Personal Information Protection Law, PIPL)~\cite{PIPL}, and found all require personal data controllers to provide some forms of disclosure to data subjects.
For example, APP Article \textit{1.3}\cite{APPs} imposes an obligation on organisational entities to \textit{``have a clearly expressed and up-to-date APP Privacy Policy about how the entity manages personal information.''}, and PIPL Article \textit{17} \cite{PIPL} stipulates that \textit{``Personal information handlers shall, before handling personal information, explicitly notify individuals truthfully, accurately, and fully of the following items using clear and easily understood language...''}

In addition to the five listed regulations, more administrations are publishing similar privacy legislation.
According to the United Nations Conference on Trade and Development (UNCTAD)~\cite{UNCTAD}, 137 out of 194 countries had put in place legislation to secure the protection of data and privacy.
%It is becoming a worldwide consensus that to raise the public awareness of privacy and to protect personal information by publishing special legislation.
Although some privacy regulations have existed since 2018, as we observe in this paper, many apps either fail to provide a privacy policy, or perfunctorily provide only a low quality privacy policy. 
APPGs are increasingly used by developers to create privacy policy for their mobile apps. 
To minimize the potential risk to breach privacy regulations, app developers need to cautiously select appropriate APPGs to generate privacy policies, and a comprehensive comparison and assessment of mainstream APPGs is essential.
Additionally, from the regulatory authorities‘ perspective, to better monitor the market and verify privacy regulations compliance, an up-to-date and in-depth empirical study on APPGs is also beneficial.


\textbf{\textit{European General Data Protection Regulation (GDPR)}}~\cite{GDPR}.
%The European General Data Protection Regulation (GDPR) \cite{GDPR} has been in effect since May 2018. 
%GDPR pioneered personal data protection legislation, and covers almost every aspect of the personal data life-cycle. 
GDPR Article \textit{12} requires that \textit{''...the controller shall take appropriate measures to provide any information referred to in Articles \textit{13} and \textit{14}...''}, where articles \textit{13} and \textit{14} specifically list \textit{``Information to be provided where personal data are collected from the data subject''}. 


\textbf{\textit{California Consumer Privacy Act (CCPA)}}~\cite{CCPA}.
%The California Consumer Privacy Act of 2018 (CCPA)  supports privacy rights and personal data integrity for California residents. 
%Businesses are required to provide prescribed information to explain their privacy practices.
In Section \textit{1798.130.(5)} and \textit{1798.135.(5)}, specific obligations include to \textit{``Disclose the following information in its online privacy policy or policies if the business has an online privacy policy...''}


\textbf{\textit{Brazilian Law of General Data Protection (LGPD)}}~\cite{LGPD}.
% \footnote{It is originally written in Portuguese}
% http://www.planalto.gov.br/ccivil_03/_Ato2015-2018/2018/Lei/L13709.htm
%The Brazilian General Data Protection Law (LGPD)  of August 2018 has obligations for data controllers and data processing within Brazil. 
Article \textit{9} requires that \textit{``The data subject has the right to facilitated access to information concerning the processing of her/his data...''}.


\textbf{\textit{Australian Privacy Principles (APP)}}~\cite{APPs}.
%The Australian Privacy Principles (APP)  in the Privacy Act of 1988, govern the collection, storage, use and disclosure of personal information.
Article \textit{1.3} imposes an obligation on organisational entities to \textit{``have a clearly expressed and up-to-date APP Privacy Policy about how the entity manages personal information.''}


\textbf{\textit{Personal Information Protection Law (PIPL) of China}}~\cite{PIPL}.
% \footnote{It is originally written in Chinese}
%The Personal Information Protection Law of the People’s Republic of China (PIPL)  protects personal information rights and interests internationally for any businesses that processes any personal data from China. 
%It came into effect in November 2021.
In Article \textit{17}, the PIPL stipulates that \textit{``Personal information handlers shall, before handling personal information, explicitly notify individuals truthfully, accurately, and fully of the following items using clear and easily understood language...''}







==> omitted_StatusQuo.tex <==
\section {Status Quo of Privacy Policy for Mobile Apps}
\label{sec_overview}

Privacy policy plays an essential role in mobile apps ecosystems. Other forms of privacy notices such as privacy nutrition labels (PNLs)~\cite{li2022understanding, zhang2022usable, zhangprivacy} focus more on providing succinct information to end users, meanwhile sacrificing in the specifics of legal elucidation. 
Privacy policy is not only required by regulations in some jurisdictions, but is also increasingly demanded by mobile app users or marketplaces. According to the App Privacy section on the Apple App Store developers page \cite{appledeveloper}, a privacy policy is required when submitting new apps or app updates.% to the Apple App Store. 

\begin{tcolorbox}
     \textit{``By adding the following links on your product page, you can help users easily access your app’s privacy policy and manage their data in your app.}
    \textit{\textbf{Privacy Policy (Required):} The URL to your publicly accessible privacy policy.''}
\end{tcolorbox}

In the Google Play Console Help Center\cite{googledeveloper}, to prepare an app for review, developers are asked to add a privacy policy that includes involved data practices:

\begin{tcolorbox}
    \textit{``Adding a \textbf{privacy policy} to your app's store listing helps provide transparency about how you treat sensitive user and device data.''}
\end{tcolorbox}
Although many principles regulate the existence and quality of privacy policies, we still discovered some critical problems in the mobile apps market, as discussed in Section~\ref{sec_overview_observation}.

\subsection{Crawled Privacy Policy Dataset}
\label{sec_overview_dataset}
To better understand the status and quality of existing privacy policies, we need a large-scale privacy policy dataset.
However, existing datasets suffer from various problems. 
% orthogonality

\textbf{The differences between datasets for previous research and our research goals.} 
Existing datasets are either not focused on mobile apps, biased, small, or outdated. First, some prior research focuses on privacy policies across all platforms, including websites and mobile apps \cite{amos2021privacy, EASE_2020, CMU_2017}, while we only target mobile apps.
Since they did not include metadata (e.g., platforms) of the collected policies, we cannot filter them out from
other platforms.
Second, some research only focus on apps of certain groups and their collected datasets are not representative enough for apps in the market.
For example, one study~\cite{USENIX_2022_GEODIFF} manually collected 5,684 ``globally popular apps.'' 
This selection criterion leads to two critical problems: 
a) The top overall popular apps appear in a limited set of categories, such as \textit{Social} and \textit{Finance}, which can drive out apps from less popular categories such as \textit{Parenting} or \textit{Libraries \& Demo}. 
b) These globally popular apps do not distribute evenly across various app categories, which may cause potential biased and unrepresentative findings.
Third, some existing datasets are small and can contain potential bias.
For example, APP-350~\cite{PETS_2019} only analysed 350 privacy policies, and another study~\cite{liu2021have} conducted fine-grained analysis on only 304 privacy policies.
% To mitigate this problem and understand the properties and potential issues in existing privacy policies, a large-scale dataset is needed. 
Finally, due to the rapid iteration of apps, apps' privacy policies, and APPGs, some prior datasets can quickly become outdated.
% Fourthly, APPGs are developed and attract increasing attentions just in recent several years, therefore 
% it is impracticable to operate our research by directly using a comparatively old dataset. Above all, considering the availability issue as well, we decide to build a new dataset that resolving all previous concerns.
As a summary, to make our findings comprehensive, generalizable, and up-to-date, we need to collect the latest large-scale dataset that can assemble apps of different popularity and from various app categories.

%, taking the absolutely and worldwide dominated place since it launched.
% There are many apps markets across Androids apps ecosystem, and Google Play Store is the largest Android apps market among them, taking the absolutely and worldwide dominated place since it launched. 
% There are 53 different categories according to Google Play Store page.  We excluded \textit{Watch apps} and \textit{Watch faces} since those are specially designed for Android smartwatches. 
% In addition, we excluded two ``fake'' categories, namely \textit{Augmented reality} and \textit{Daydream}, because the contained apps actually belong to another app category as shown on their Google Play homepages. (Note that one app can only belong to one category at Google Play Store.) 
% we found two ``fake'' categories namely \textit{Augmented reality} and \textit{Daydream}, because apps from these two categories actually belong to another category based on the information on their homepages (Note that one app can only belong to one category at Google Play Store.). 
% This can also be verified by their internal web address structure. The hyperlink of \textit{Augmented reality} is ``.../apps/stream/baselist\_featured\_arcore'', while the hyperlinks for \textit{Finance} and \textit{Social} are ``.../apps/category/FINANCE'' and ``.../apps/category/SOCIAL'' respectively. 
% Finally, we obtained 17 game categories and 32 non-game categories. 
% This also can be verified by https://support.google.com/googleplay/android-developer/answer/9859673?hl=en#zippy=%2Capps%2Cgames

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/distribution.pdf}
%   \caption{Apps distribution across 49 categories at Google Play Store.}
%   \label{fig_distribution}
% \end{figure}

\textbf{Google Play Store.} 
It has been widely discussed and recognized that Android mobile apps are more transparent and friendly to academic research compared to iOS mobile apps \cite{habchi2017code, kollnig2021iphones}. 
There are many app markets for the Android platform, but Google Play is the largest and the most accessible app market, with over two million apps, according to AppBrain~\cite{appbrain}. Thus, we only focus on the Google Play Store.
Particularly, we noticed some apps are specially designed for Android smartwatches instead of mobile phones; therefore, we excluded apps belonging to categories named \textit{Watch apps} and \textit{Watch faces}.

\textbf{Our dataset.}
Above all, we collected a new large-scale privacy policy dataset from existing apps on the Google Play Store.
We collected app metadata from AndroZoo~\cite{Allix:2016:ACM:2901739.2903508}, which is a large-scale and growing Android app collection extracted from multiple sources, including the Google Play Store.
We removed duplicates and apps from other app markets and then randomly sampled 268,500 apps as our initial app dataset, which is around 10\% of the whole app population.
From this initial sample, we observed that some apps are either invalid or not usable.
These were mainly dummy apps or student apps with a package size normally less than 10 KB, so we removed invalid apps like these.
We excluded unavailable apps that returned error messages on their Google Play Store page. 
Apps can be unavailable for many reasons including geodifferences \cite{USENIX_2022_GEODIFF} caused by government censoring, or being removed by Google because of disruptive adware, malware, restricted content, or other reasons.
%Developers can also unpublish or disable their own apps. 
After these exclusions, we were left with 99,194 usable apps and their metadata. 
We then used ``google play scraper'' \cite{googleplayscapper} to obtain app information including privacy policy links, app categories showed, required device permissions, etc.
Based on the available privacy policy links shown on app's homepages, we further utilize the \textit{BeautifulSoup}~\cite{beautifulsoup} and \textit{Selenium}~\cite{Selenium} python packages to download those websites.
Eventually, we obtained 46,472 privacy policies, and we refer to this privacy policy dataset as \textbf{``Crawled Privacy Policy Collection.''}~\footnote{It is available at: 
https://github.com/APPG-APPG/APPG.}
We conducted the above data gathering process in March 2022.
%Among these unavailable apps, xxx no longer exist in the market because of the change of app package names, withdrawal by app developers or removal by google, xxx could not be accessible due to the geodifferences %\cite{USENIX_2022_GEODIFF} caused by government censoring.

% Apps that are not from Google Play Store are filtered out, and duplicates samples are removed from the dataset. Moreover, 
% apps whose apk size are less than $1KB$ are deleted as well, since they are not regarded as valid and usable apps. 
% Then we randomly sample 268,500 apps, which is around 5\% of the whole apps population. 
% We use ``google play scraper \footnote{https://pypi.org/project/google-play-scraper/} to crawl apps from Google Play Store, and we set language is English and country is Australia. 
% Eventually we obtained 99,194 available apps and their metadata, unavailable apps return the error message \textit{``We're sorry, the requested URL was not found on this server.''} on its Google Play Store page. This problem could be caused by many potential reasons, such as geodifferences \cite{USENIX_2022_GEODIFF} caused by government censoring, or removed by Google because of disruptive adware, malware, clone apps and plagiarism, restricted content, etc. Moreover, the developers could unpublish or disable their own apps.

\subsection{Observations on Status Quo}
\label{sec_overview_observation}
In this section, we report an analysis of app privacy policies and identify three common problems in existing apps: missing/unavailable privacy policies, low quality privacy policies, and language non-localization problems.
Although similar problems were discussed in several previous studies~\cite{PETS_2019, USENIX_2022_GEODIFF, li2022understanding}, considering the rapid development of markets, we believe it is worthwhile to revisit those critical issues.
% report some discussions and analysis based on the dataset we obtained from Google Play Store. Specifically, based on the privacy policy links at the \textit{``ADDITIONAL INFORMATION''} section on their Google Play Store homepages, we utilize Selenium \cite{Selenium} python package to crawl privacy policies for 99,194 available apps.

\subsubsection{Missing Links and Unavailable Privacy Policies}
\label{sec_observation_missing}

% \jieshan{may discuss installation number/rating}
%In addition, we also conduct a correlation test (i.e., calculating the Kappa value) to measure the correlations between installation number/rating and missing rate. The result indicates that there is ?? relationship between these two factors.. 

We observed that 15.7\% (15,572/99,194) of apps do not provide a privacy policy link on their Google Play Store homepage.
One prior study~\cite{PETS_2019} reported that this statistic was 49.1\% in 2019. 
Seemingly, as more regulation principles were launched, and more law enforcement efforts were practiced, fewer apps provided a privacy policy.
% However, another prior study of ``globally popular apps''~\cite{USENIX_2022_GEODIFF} reported that only 76 out of 5385 (1.4\%) apps did not a provide privacy policy links in 2021. 
However, we found that 37.5\% (37,150/99,194) of privacy policy links lead to unavailable websites with error messages such as ``403 Forbidden'' or ``404 Not Found.''
This problem could be caused by potential reasons such as deliberately providing a dummy link, an outage, or the removal of the website server.
Hence, in addition to simply requiring app developers to provide the privacy policy, the mobile app market also needs to frequently and regularly verify the validity of provided privacy policy links.


\subsubsection{Low Quality Privacy Policies}
\label{sec_observation_lowquality}

% After manually inspecting hundreds of privacy policies in the dataset, we found dozens of quasi privacy policies. 

Several previous studies~\cite{liu2021have, PETS_2019} reported that it was not rare that some apps only provide a low quality privacy policy, and we spotted a similar issue in our dataset.
Firstly, we noticed that some privacy policies do not contain meaningful privacy-related context, or are just  dummy websites.
For example, ``Bway App'' is a free app that provides football results, football statistics, trends, and match result predictions, with over 10,000 installs; however, their privacy policy website~\cite{BwayApp} does not contain any content. Moreover, the file size of the crawled privacy policy website is close to 0 KB.
In addition, some are apparent ``homemade'' privacy policies that are too general to include essential data practices.
For instance, ``Easy Communication'' is designed to help people with autism, cerebral palsy, dyslexia, intellectual disability, and other special needs to communicate easily, with over 1,000 installs. Its privacy policy~\cite{EasyCommunication} only has 156 words, and ambiguously mentions permissions without any elaborations.
Based on our observations and previous work, we empirically set the file size threshold as 2 KB~\cite{liu2021have}, and the document length threshold as 200 words~\cite{USENIX_2022_GEODIFF}. If a crawled privacy policy does not meet both criteria, it will be regarded as a low quality privacy policy.
We identified 22.3\% (10,375/46,472) low quality privacy policies in total.

% Less installs also need to be paid attentions?
% Figure~\ref{quality_boxplot} shows the comparison between apps with a low quality and a high quality privacy policies. 
% In terms of installs, we can see that apps with a high quality privacy policy have more installs, and the 75\% quartile reaches around 10,000, which is around as twice many as the installs of apps with a low quality privacy policy. 
% The reason why the scores are close is that an app would be officially rated only if it receives a decent amount of reviews, and apps with low quality privacy policy usually would not be qualified to receive a score.
% \vspace{-0.1cm}
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.0\linewidth]{Figures/quality_boxplot.png}
%   \vspace{-10pt}
%   \caption{Number of installations and ratings of apps based on the quality of privacy policies}
%   \label{quality_boxplot}
% \end{figure}
% \vspace{-0.1cm}


\subsubsection{Language non-Localization Problem}
\label{sec_observation_language}
Language localization is necessary to promote apps in a global market. 
Although app UI and content may be translated, app developers may neglect the privacy policy. 
We employed the Python package \textit{langdetect}~\cite{langdetect} to detect the language of crawled privacy policy documents and found 20.5\% (9,523/46,472) of apps do not provide an English privacy policy, although these apps were released in markets where the primary language is English. 
We observed this problem even with top apps from some large companies. 
For the privacy policies of the top 1,000 most installed apps (all $>$ 500k installs) in our dataset, there are still around 14.1\% of them that do not provide an English privacy policy.
APPGs may be a solution to language non-localization problems. 
Although currently only APPG \#1 \textit{Iubenda} supports multilingual generation, some APPGs (\#4, \#7, and \#9) have included placeholders for future options for language selection.



% --------------------------------------------%
% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/problem-category-proportion.pdf}
%   \caption{Apps distribution across 49 categories at Google Play Store.
%   \jieshan{(1)Please enlarge the legend and the label of y-axis. May consider adding texts showing some extreme values. (2) For game categories, please add ``Game'' before their exact type. For example, for action category, change it to Game\_Action. (3) This figure is hard to understand. May find a better method to show the info}. 
%   }
%   \label{fig_problems_distribution}
% \end{figure*}

% \begin{table}[h]
% \label{}
% \caption{The top 5 categories that suffer three observed problems.}
% \centering
% \begin{tabular}{|l|l|l|} 
% \hline
% \multicolumn{3}{|c|}{\textbf{Top 5 categories of missing privacy policy links}}                                    \\ 
% \hline
% \textbf{category} & \textbf{\textbf{\% has the problem}} & \textbf{\textbf{\# has the problem}}  \\ 
% \hline
% Game\_Arcade      & 31.2\%                                   & 717                                  \\
% Libraries \& Demo   & 30.3\%                                   & 60                                   \\
% Game\_Adventure   & 25.2\%                                   & 232                                  \\
% Game\_Board       & 24.2\%                                   & 112                                  \\
% Game\_Casual      & 24.0\%                                   & 570                                  \\
% \hline
% \end{tabular}

% \smallskip
% \noindent
% \begin{tabular}{|l|l|l|} 
% \hline
% \multicolumn{3}{|c|}{\textbf{Top 5 categories of low quality privacy policies}}                                    \\ 
% \hline
% \textbf{category} & \textbf{\textbf{\% has the problem}} & \textbf{\textbf{\# has the problem}}  \\ 
% \hline
% Event      & 32.9\%                                   & 79                                  \\
% Sports   & 27.6\%                                   & 37                                \\
% Game\_Sports   & 27.2\%                                   & 104                                 \\
% Maps \& Navigation       & 27.2\%                                   & 369                                 \\
% Music \& Audio      & 27.0\%                                   & 212                              \\
% \hline
% \end{tabular}

% \smallskip
% \noindent

% \begin{tabular}{|l|l|l|} 
% \hline
% \multicolumn{3}{|c|}{\textbf{Top 5 categories of privacy policy language non-localized}}                                    \\ 
% \hline
% \textbf{category} & \textbf{\textbf{\% has the problem}} & \textbf{\textbf{\# has the problem}}   \\ 
% \hline
% News \& Magazines      & 42.0\%                                   & 389                                \\
% Maps \& Navigation   & 35.9\%                                   & 248                                  \\
% Shopping   & 35.5\%                                   & 577                                 \\
% Food \& Drink      & 32.9\%                                   & 538                                 \\
% Auto \& Vehicles     & 32.0\%                                   & 114                                 \\
% \hline
% \end{tabular}

% \end{table}

